POLYRAG: Integrating Polyviews into Retrieval-Augmented Generation for Medical Applications

Large language models (LLMs) have become a disruptive force in the industry, introducing unprecedented capabilities in natural language processing, logical reasoning and so on. However, the challenges of knowledge updates and hallucination issues have limited the application of LLMs in medical scenarios, where retrieval-augmented generation (RAG) can offer significant assistance. Nevertheless, existing retrieve-then-read approaches generally digest the retrieved documents, without considering the timeliness, authoritativeness and commonality of retrieval. We argue that these approaches can be suboptimal, especially in real-world applications where information from different sources might conflict with each other and even information from the same source in different time scale might be different, and totally relying on this would deteriorate the performance of RAG approaches. We propose PolyRAG that carefully incorporate judges from different perspectives and finally integrate the polyviews for retrieval augmented generation in medical applications. Due to the scarcity of real-world benchmarks for evaluation, to bridge the gap we propose PolyEVAL, a benchmark consists of queries and documents collected from real-world medical scenarios (including medical policy, hospital & doctor inquiry and healthcare) with multiple tagging (e.g., timeliness, authoritativeness) on them. Extensive experiments and analysis on PolyEVAL have demonstrated the superiority of PolyRAG.

==> sec-limits.tex <==
\section{Limitations}\label{sec:limits}
In this section, we aim to provide a comprehensive overview by systematically outlining the limitations and constraints inherent to our research, thereby facilitating a deeper understanding of the scope and potential boundaries of our findings. Here we present these considerations below in a detailed manner, encouraging further discussion and guiding future studies to build upon our work with enhanced awareness and insights.

\subsection{Limitations of Utility Model}
Initially, it is crucial to underscore that the efficacy of the proposed utility model is profoundly dependent on the robust guidance provided by a high-performant large language model (LLM). Our investigations have indeed revealed that an LLM with modest parameters, such as LLama 7B or 13B, suffices to train a utility model that is capable of meeting satisfactory performance standards, which underscores the feasibility of deploying moderately sized LLMs for this purpose without necessitating available models of quite large scale.

Furthermore, to guarantee the seamless operation of the selective retrieval mechanism, it is imperative that the LLM employed for executing the end-task possesses comparable, if not superior, capabilities to the one in the utility model's training phase. The rationale behind this requirement lies in the need for a deep understanding and contextual precision during the retrieval process, which can only be assured by an LLM that is at least as competent as the the one used for utility model training. Any deviation from this, i.e., utilizing a weaker LLM for the final task, risks undermining the efficacy of the selective retrieval process, potentially leading to sub-optimal results or performance degradation. 


\subsection{Limitations in Super-Long Contexts of Specialized Domains}
Expanding upon our initial point, our research introduces a fresh perspective that rejuvenates the discourse on retrieval-augmented content generation of commonsense knowledge. It spotlights the potential for more sophisticated integration of information retrieval within generative models. However, it also acknowledges the existence of a significant gap in handling intricate real-world scenarios of specialized domains such as finance, law, and medicine where an extensive volume of text documentation, must be comprehensively analyzed before formulating a response. These domains necessitate a profound understanding derived from dense and lengthy materials that require domain knowledge, presenting challenges unaddressed by current methodologies.

\paratitle{Future Work.} One of the pivotal directions for future development entails enhancing our framework to excel in managing super-long contexts in specialized domains. This endeavor aims to equip our model with the capability to navigate, interpret, and synthesize information from vast corpora that requires domain knowledge, thereby transcending the limits of existing systems and ushering in a new era of advanced text generation across complex disciplines.



\subsection{Limitations in Industrial Applications}
The cornerstone in retrieval-augmented generation is the reliance on meticulously augmented information, acting as the key point for generating contextually rich and accurate responses. In our empirical investigations, we strategically integrated datasets meticulously curated by humans together with high-quality retrieval data sources like Wikipedia. This approach was instrumental in validating the efficacy of our proposed model, underscoring the importance of high-caliber data inputs for achieving superior outcomes. Nonetheless, transitioning from controlled experimental environments to the pragmatic realms of industrial applications, such as search engines, unveils a new set of challenges. Here, the input queries might be ambiguous, poorly structured, or even incomprehensible, significantly challenging the retrieval mechanism. Compounding this issue, the data sources tapped into can often be of questionable veracity or riddled with inaccuracies or even inconsistencies, \eg clickbait  websites, rendering the verification of retrieved information a daunting task. 

\paratitle{Future Work.} Real-world industrial applications of retrieval-augmented generation faces substantial challenges such as ambiguous queries and unreliable data sources, which urges techniques for enhancing system robustness and reliability. In the future, we hope to focus more on intelligent query interpretation, real-time data validation, and adaptability to evolving information landscapes to advance the applicability of retrieval-augmented generation in more complex scenarios.

